Impact of Multi-connectivity on Channel Capacity and Outage Probability in Wireless Networks

Multi-connectivity facilitates higher throughput, shorter delay, and lower outage probability for a user in a wireless network. Considering these promises, a rationale policy for a network operator would be to implement multi-connectivity for all of its users. In this paper, we investigate whether the promises of multi-connectivity also hold in such a setting where all users of a network are connected through multiple links. In particular, we consider a network where every user connects to its k closest base stations. Using a framework of stochastic geometry and probability theory, we obtain analytic expressions for per-user throughput and outage probability of $k$-connectivity networks under several failure models. In contrast to the conclusions of previous research, our analysis shows that per-user throughput decreases with increasing k. However, multi-connected networks are more resilient against failures than single connected networks as reflected with lower outage probability and lead to higher fairness among the users. Consequently, we conclude that rather than implementing multi-connectivity for all users, a network operator should consider it for its users who would benefit from additional links the most, e.g., cell edge users.

==> IEEEtran/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> removed.tex <==
\subsubsection{Deterministic overload failure}
We assume that base stations fail if the degree of this base station is higher than $N$. This means that the probability that a link fails is equal to the probability that the size-biased degree is higher than $N$:
\begin{IEEEeqnarray}{rCl}
    \E(p) &=& \P(D_{BS}^* \geq N) = \frac{1}{k \lambda} \sum_{n=N}^\infty n\cdot \P(D_{BS} = n) \nonumber \\
    &=&\frac{1}{k\lambda} \tk \sum_{n = N}^\infty \frac{\Gamma(n+a_k)}{\Gamma(a_k)\Gamma(n)} \left(\frac{\lambda k}{\lambda k + a_k}\right)^n \nonumber \\
    &=& \frac{1}{k \lambda} \tk \frac{\Gamma(N + a_k)}{\Gamma(a_k)\Gamma(N)} \left(\frac{\lambda k}{\lambda k + a_k}\right)^N \nonumber \\
    &&_2 F_1\left(1, N + a_k, N, \frac{k \lambda}{k\lambda + a_k}\right).
\end{IEEEeqnarray}

The expected channel capacity is:
\begin{IEEEeqnarray}{rCl}
    \E(C_{sum}) &=& (1-\E(p)) \sum_{j=1}^k \E\left( C_j\right) \nonumber\\
    &=& \frac{\overline{\wtot}}{k \lu} \Bigg(1 -  \frac{1}{k \lambda} \tk \frac{\Gamma(N + a_k)}{\Gamma(a_k)\Gamma(N)} \left(\frac{\lambda k}{\lambda k + a_k}\right)^N\nonumber \\
    && _2F_1\left(1, N + a_k, N, \frac{k \lambda}{k\lambda + a_k}\right)\Bigg) \sum_{j=1}^k \E(\log_2(1+SNR_j).
    \IEEEeqnarraynumspace\label{eq:overload_det_failure}
\end{IEEEeqnarray}

\subsubsection{Proportional distance failure}
When failures happen with a probability proportional to the length of the link, we can express this as:
\begin{IEEEeqnarray}{rCl}
    p_j = \begin{cases}
        0, \hspace{3cm}& R_j \leq 1,\\
        1 -  R_j^{-\beta}, &R_j > 1,
    \end{cases}
\end{IEEEeqnarray}
for a constant $\beta$.

We can again find the expected channel capacity \eqref{eq:channel_capacity_with_failure}:
\begin{IEEEeqnarray}{rCl}
    \E(C_{sum}) 
    &=& \frac{\overline{\wtot}}{k \lu} \sum_{j=1}^k  \E\left( R_j^{-\beta}\log_2(1+cR_j^{-\alpha})\right)
\end{IEEEeqnarray}

\begin{IEEEeqnarray}{rCl}
    \E(C_{sum}) &=& \frac{\overline{\wtot}}{k \lu}\sum_{j=1}^k \E\left((1 - p_j) \log_2(1+SNR_j)\right) \nonumber \\
    &=& \frac{\overline{\wtot}}{k \lu} (\lbs \pi)^{\frac{\beta}{2}}\sum_{j=1}^k \frac{\Gamma\left(j-\frac{\beta}{2}\right)}{\Gamma(j)} \E(\log_2(1+SNR_j). \IEEEeqnarraynumspace
\end{IEEEeqnarray}

The outage probability is
\begin{IEEEeqnarray}{rCl}
    \P(D_U = 0)&=& \prod_{j=1}^k \left( 1 - (\lbs \pi)^{\frac{\beta}{2}}  \frac{\Gamma(j - \frac{\beta}{2})}{\Gamma(j)}  \right) 
\end{IEEEeqnarray}

==> table_of_notations.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{c|c}
        SC      &   Single-connectivity \\
        MC      &   Multi-connectivity  \\
        LoS     &   Line of Sight\\
        PPP     &   Poisson Point Process\\
        $\lbs, \lu$  &   Density of base stations/users\\
        $\lambda$   &   Amount of users per base station\\
        $N_{BS}, N_U$   &   Number of base stations/users\\
        $D_{BS}, D_U$   &   Number of links to a base station/user (degree)\\
        $C_j$           &   Channel capacity of base station $j$\\
        $W_j$           &   Bandwidth that a base station uses\\
        $W_{tot}$       &   Total bandwidth of the network\\
        $\overline{\wtot}$  &   Total bandwidth per area\\
        $SNR_j $    &   Signal-to-noise-ratio of base station $j$\\
        $p$     &   Power of a base station \\
        $\sigma$    &   Noise of a base station\\
        $c$     & $\frac{p}{\sigma}$ \\
        $\alpha$    & Path loss exponent, $2 \leq \alpha \leq 4$\\
        $\phi$  & $\lbs \pi c^{\frac{2}{\alpha}}$\\
        $R_j$   & Distance to base station $j$\\
        $\Gamma(s,x)$   & Upper incomplete gamma function \\
        $_pF_q(a,b,x)$  & Hypergeometric function\\
        
        
    \end{tabular}
    \caption{Table of notations}
    \label{tab:my_label}
\end{table}
